PSENet: Progressive Self-Enhancement Network for Unsupervised Extreme-Light Image Enhancement

The extremes of lighting (e.g. too much or too little light) usually cause many troubles for machine and human vision. Many recent works have mainly focused on under-exposure cases where images are often captured in low-light conditions (e.g. nighttime) and achieved promising results for enhancing the quality of images. However, they are inferior to handling images under over-exposure. To mitigate this limitation, we propose a novel unsupervised enhancement framework which is robust against various lighting conditions while does not require any well-exposed images to serve as the ground-truths. Our main concept is to construct pseudo-ground-truth images synthesized from multiple source images that simulate all potential exposure scenarios to train the enhancement network. Our extensive experiments show that the proposed approach consistently outperforms the current state-of-the-art unsupervised counterparts in several public datasets in terms of both quantitative metrics and qualitative results. Our code is available at https://github.com/VinAIResearch/PSENet-Image-Enhancement.

==> sections/1_introduction.tex <==
\section{Introduction}

% \khoi{main idea: even we do not know how to enhance the given image but we know how good a region looks like based on the three metrics, so we randomly sample multiple references with different brightness values, compare, and combine them together pixel by pixel, resulting in the best combination to use as the pseudo GT image.}


Producing images with good contrast, vivid color, and rich details is an important goal of computational photography. However, acquiring such pleasing images is not always a trivial task because of harsh lighting conditions, including extreme low lighting or unbalanced lighting conditions caused by backlighting. The resulting under-/over-exposed images usually decrease not only human satisfaction but also computer vision system performance such as object detection or image segmentation~\cite{Rashed_2019, tan2020nighttime}. Exposure problems occur early in the capturing process and are difficult to fix after the final 8-bit image has been rendered. This is because the camera image signal processor uses highly nonlinear operations to create the final 8-bit standard RGB image~\cite{karaimer2016software}. 
% Even for well-established image enhancement software, correcting degraded images is still a difficult task.

\begin{figure}[t]
\includegraphics[width=\textwidth, page=1]{image/figure.pdf}
\caption{Visual comparison on an over-exposed scene. Most of previous state-of-the art failed to recover the over-exposed case except recent work proposed by by Afifi \etal{}~\cite{afifi2021learning}, which is trained in a supervised fashion.}
\label{fig:teaser}
\end{figure}

Many recent works have mainly focused on under-exposure cases where images are often captured in low-light conditions (\eg{} nighttime). These works have achieved promising results for enhancing the quality of images even captured under extreme low-light conditions. 
However, they failed to handle over-exposure images, as shown in Figure~\ref{fig:teaser}. The recent work proposed by Afifi \etal{}~\cite{afifi2021learning} achieves impressive results in improving both under- and over-exposed cases. However, their proposed method is designed to work in a supervised manner which requires a large dataset of wrong-exposed and corresponding ground-truth (GT) well-exposed image pairs. This data collecting is typically time-comsuming and expensive.
% Furthermore, their proposed network is heavy, which is not suitable for edge devices (\eg{} smartphones). 


%In this paper, our goal is to develop a robust image enhancement framework for handling a variety of lighting conditions, including both under- and over-exposed cases. This framework needs to be trained in an unsupervised manner so that it removes the burden of collecting pixel-wisely paired wrong-exposed and ground truth well-exposed images under controlled environments in large scale and diversities. In addition, this method should be lightweight enough to install and run real-time on edge devices. Our main idea is to divide the original complicated space into multiple small and separate subspaces to reduce the need of a big and complicated model.


In this paper, we propose a novel unsupervised approach which does not require any well-exposed GT images. The key idea is to generate a pseudo GT image given the input wrong-exposed one in order to train an enhancement network. The pseudo GT image across training epochs is progressively generated by choosing the visually best regions taken from multiple sources including the output of the same input image from the previous epoch, the brighter/darker reference images by changing gamma value of the input image, and the input image itself. The choosing criteria are well-exposedness, local contrast, and color saturation, which are driven by human knowledge of a visually good image and have been shown to be effective in measuring perceptual image quality~\cite{mertens2007exposure}. In this way, the task of generating pseudo GT images is simply comparing and selecting the best regions from different sources where almost all possible cases of exposure are simulated in training. Furthermore, by using the output of the previous epoch as a source for choosing, we ensure that the output of the current epoch will be better than or at least equal to that of the previous one, giving the name of our approach \Approach~-- Progressive Self Enhancement Network.


% In this paper, we propose a novel two-branch framework where the first branch is to synthesize pseudo high-quality ground-truth images for training while the second branch is to enhance its quality. \rang{need to justify why it help to handle over-exposure, and link to SURE} These two branches are combined in an unsupervised manner. In addition, a tone mapping based on the gamma correction is adopted in the second branch to enhance the overall image contrast. We also propose a new set of unsupervised loss functions to drive the learning process. Experimental results validate our method not only improves the brightness of an image but also increases its contrast and visibility. 
% 
Our contributions are summarized as follows:
\begin{itemize}
    % \item We proposed a novel two-branch framework for addressing a variety of lighting conditions. Our proposed framework is designed to work in an unsupervised manner so as to remove the burden of collecting the paired images. 
    \item We introduce a new method for generating effective pseudo-GT images from given wrongly-exposed images. As a result, the burden of gathering the matched image pairs is removed. 
    
    \item We propose a novel unsupervised progressive pseudo-GT-based approach that is robust to a wide range of severe lighting conditions, including under-exposure and over-exposure.
    
    \item Comprehensive experiments are conducted to show that our approach outperforms previous unsupervised methods by large margins on SICE \cite{sice} and Afifi \cite{afifi2021learning} datasets and obtains comparable results with supervised counterparts.
    
    % \item Importantly, our lightweight method can process 14 FPS on mobile devices, which is up to 7x faster compared with the previous state-of-the-art.
\end{itemize}


==> sections/2_relatedwork.tex <==
\section{Related Work}
Image enhancement approaches can be divided into two categories based on the algorithm principle: traditional methods and learning-based methods.

\noindent\textbf{Traditional methods.} One of the simplest and fastest approaches is transforming single pixels of an input image by a mathematical function such as linear function, gamma function, or logarithmic function.  For example, histogram equalization-based algorithms stretch out the image's intensity range using the cumulative distribution function, resulting in the image's increased global contrast. Retinex theory~\cite{retinexTheoryLand}, on the other hand, argues that an image is made from two components: reflectance and illumination. By estimating the illumination component of an image, the dynamic range of the image can be estimated to reproduce images with better color contrast. However, most Retinex algorithms use Gaussian convolution to estimate illumination, thus leading to blurring edges \cite{exprimentbasedreview}. Frequency-domain-based methods, by contrast, preserve edges by employing the high-pass filter to enhance the high-frequency components in the Fourier transform domain \cite{homomorphicFilter}, or by decomposing the input image and then suppressing the low-frequency components and enhancing the high-frequency ones \cite{exprimentbasedreview}. However, the adaptability of such traditional methods is often limited due to their unawareness of the overall and local complex gray distribution of an image \cite{exprimentbasedreview}. For a systematic review of conventional approaches, we suggest readers refer to a recent work of Wang \etal{} \cite{exprimentbasedreview}. 

\noindent\textbf{Learning-based methods.} In recent years, there has been increasing attention to learning-based photo enhancing methods in both supervised and unsupervised approaches.

\noindent\textit{Supervised learning} methods aim to recover natural images by either directly outputing the high quality images ~\cite{lore2016llnet},~\cite{Lv2018MBLLENLI},~\cite{Li2020LuminanceawarePN},~\cite{Xu2020LearningTR} or learning specific parameters of a parametric model (\eg{} Retinex model)~\cite{},~\cite{hdrnet},~\cite{DeepUPE},~\cite{moran2020deeplpf} from a paired dataset.
SID~\cite{SeeInTheDark} is a typical example in the first direction. In this work, the authors collect a short-exposure low-light image dataset and adopt a vanilla Unet architecture \cite{ronneberger2015unet} to produce an enhanced sRGB image from raw data thus replacing the traditional image processing pipeline. Following this work, Lamba and Mitra~\cite{RealTimeDarkImageRestorationCvpr2021} present a novel network architecture that concurrently processes all the scales of an image and can reduce the latency times by 30\% without decreasing the image quality. Different from the previously mentioned approaches, Cai \etal{}~\cite{sice} explore a new direction in which both under- and over-exposed images are considered. They introduce a novel two-stage framework trained on their own multi-exposure image dataset, which enhances the low-frequency and high-frequency components separately before refining the whole image in the second stage. Afifi \etal{}~\cite{afifi2021learning} put a further step in this direction by introducing a larger dataset along with a coarse-to-fine neural network to enhance image qualities in both under- and over-exposure cases. For learning a parametric model, Retinex theory~\cite{Land1971LightnessAR} is often adopted~\cite{retinexnet, Li2018LightenNetAC, DeepUPE}. Benefiting from paired data, the authors focus on designing networks to estimate the reflectance and illumination of an input image. Dealing with the image enhancement task differently, HDRNet~\cite{hdrnet} present a novel convolutional neural network to predict the coefficients of a locally-affine model in bilateral space using pairs of input/output images.


\begin{figure*}[ht]
\centering
\includegraphics[width=\textwidth]{image/main_diagram.pdf}
\caption{Overview of our proposed framework which comprises three main modules: reference image generator, pseudo GT image generator, and enhancement network. Given the input image $I$, the reference image generator randomly generates multiple reference images with different exposure values, half of them which are brighter than the input image while the rest are darker. The pseudo GT image generator then takes the input image, the output image from the previous epoch, and the generated reference images as input to produce the pseudo GT image $T$ which is visually better than each of the input components alone based on the three proposed scoring criteria. Finally, the enhancement network predicts the gamma map $\gamma$ to combine with the original image $I$ to obtain the output image $Y$. The enhancement network is trained with two loss functions: reconstruction loss between the output image $Y$ and the pseudo GT image $T$, and the total variation loss applied on the predicted gamma map $\gamma$ to imply the smoothness in prediction. It is worth noting that only the enhancement network is used in testing.}
\label{fig_framework-overview}
% \vspace{-5pt}
\end{figure*}

\noindent\textit{Unsupervised learning.} Collecting paired training data is always time-consuming and expensive. To address this issue, an unpaired GAN-based method named EnlightenGAN is proposed in~\cite{enlightengan}. The network, including an attention-guided U-Net as a generator and global-local discriminators, shows promising results even though the corresponding ground truth image is absent. To further reduce the cost of collecting reference ground truth images, a set of methods~\cite{Zhang2019ZeroShotRO, Zhu2020ZeroShotRO, zerodce, dce_extension} that do not require paired or unpaired training data are proposed. Two recent methods in this category named ZeroDCE~\cite{zerodce} and Zheng and Gupta~\cite{semanticguided} show impressive results in low-light image enhancement tasks by using a CNN model trained under a set of no reference loss functions to learn an image specific curve for producing a high-quality image. However, their methods seem to perform poorly when extending to correct overexposed images, as shown in Figure~\ref{fig:teaser}.



Most of the previous approaches mainly focused on low light images. There are only few methods~\cite{hdrnet, sice, afifi2021learning} attempting to deal with both under and overexposed images, but all of them are supervised. Our proposed method, in contrast, is the first deep learning work handling these extreme lighting conditions in an unsupervised manner.
% \textit{Supervised learning} methods aim to estimate the intermediate parameters for the proposed model. For example, Retinex based methods~\cite{KinDZhang, retinexnet} attempt to learn the reflectance and illumination of the image.  HDRNet by Gharbi et al.~\cite{hdrnet} is a combination of guided upsampling and bilateral grid, which learns a grid of affine coefficients using convolutional neural network (CNN) . Inheriting the idea of bilateral grid application, Wang et al. proposed DeepUPE~\cite{DeepUPE} which predicts the multi-channel illumination component via CNN. According to Zeng et al.~\cite{zeng2020lut}, most of the enhancement modules in practical systems employ a common technique which is 1-dimensional or 3-dimensional lookup tables (1D or 3D LUTs), the authors stated that using a small CNN to tune these LUTs instead of fixing them manually improves both expressiveness and flexibility of photo enhancement. Image-to-image translation methods aim to learn the parameters mapping from one image to another directly. Steffens et al.~\cite{ReExposeNet} adapted the idea of U-net and present ReExpose-net, which maximize signal and feature recovery on low-light images . A variety of generative adversarial network (GAN) based models have been proposed for the image synthesis and translation \cite{enlightengan}. Not until EnlightenGAN was published did it become the first unsupervised and one-path GAN based model for the low-light image enhancement task \cite{enlightengan}.

% \textit{Reinforcement learning} methods try to imitate the process of image retouching. White-Box by Hu et al.~\cite{whitebox} use reinforcement learning guided by a GAN to learn the parameters for a series of resolution-independent filters. Park et al.~\cite{DeepQNet} assumed the enhancement process is a Markov Decision Process where action is the global color adjustment operations and trained the Deep Q-Network to select their parameters. Recent great work by Afifi et al.~\cite{afifi2021learning} delivers impressive results in improving both under- and over-exposure scenarios. Their proposed solution, on the other hand, is designed to work in a supervised manner, which necessitates a huge dataset of degraded and non-degraded image pairs. In contrast, our proposed method in this paper is the first deep learning work handling the extreme lighting conditions in an unsupervised manner. 

% \textit{Unsupervised learning} methods .Yi et al. proposed ZeroDCE~\cite{zerodce}, an unsupervised method, learns a set of parameters for its nonlinear mapping functions.


%\noindent\textbf{Datasets.} Public datasets play a key role  in learning-based methods. Various datasets have been published for the paired low-light image enhancement task since the MIT-Adobe FiveK in 2011. Other paired datasets have been published e.g. LOw-Light (LOL) contains low-/normal-light image pairs and was released along with RetinexNet \cite{retinexnet}. See-in-the-Dark (SID) dataset contains raw and long-exposure image pairs \cite{SeeInTheDark}. Recent works have been focusing on contrast enhancement rather than under-exposed images, which means it should also deal with over-exposed images. Cai et al. proposed the SICE dataset, which contains multi-exposed images and their corresponding high-quality reference images \cite{sice}. Additionally, Afifi et al. introduced a multi-exposed paired dataset rendered from the MIT-Adobe FiveK \cite{afifi2021learning}.


==> sections/3_method.tex <==
\section{Methodology}
Given an sRGB image, $I$, captured under a harsh lighting condition with low contrast and washed out color, our approach aims to reconstruct the corresponding enhanced image, $Y$, which is visibly better and visually pleasant in terms of contrast and color without any supervision. 
% Based on the key idea is that defining a metric to compare the quality of two images is easier than defining a function to measure how visually good an image is, 
% 
To address the problem, our key contribution is to propose a new self-supervised learning strategy for training the image enhancement network. That is, we randomly synthesize a set of reference images to be combined together to produce a synthetically high-quality ground-truth image for training. The way of combination is driven by the human knowledge of how visually good an image is.
% new image enhancement framework, in which we randomly synthesize a set of reference images, and combine them to create a synthetically high-quality ground-truth image. This image is then used to guide our enhancement network to improve the quality of the input image. 

First, our reference generator takes as input an image and generates $2N$ images where the first $N$ images have lower brightness and the others have higher brightness compared to the input image. Then, the pseudo ground truth generator module uses these generated images along with the input and the previous prediction of the enhancement network to create a pseudo-ground-truth image. It is worth noting that including the previous prediction in the set of references ensures that the quality of pseudo-ground-truth image is greater or at least equal to the current prediction, thus making our training progressively improved. Our training framework is illustrated in Figure~\ref{fig_framework-overview} and the detail of each module will be described in the following sections.

\subsection{Random Reference Image Generation} \label{refence_generator}

% In this stage, we generate $2N$ reference images, with $N$ images being the underexposed version of input image $I$ and $N$ images being the overexposed version of $I$. 

To synthesize an under/over-exposed image, we employ a gamma mapping function, which is a nonlinear operation often used to adjust the overall brightness of an image in the image processing pipeline \cite{gamma_def}. The gamma mapping function is based on the observation that human eyes perceive the relative change in the light following a power-law function rather than a linear function as in cameras \cite{krueger1989reconciling}. The connection between the gamma mapping function and the human visual system enables the gamma mapping function to be widely used in image contrast enhancement~\cite{5370400, rahman2016adaptive,7868607}. However, rather than apply gamma function directly to the original image, we apply it to the inverted image to generate $2N$ reference images $Y_n$ as follows: 
\begin{equation}
    Y_n = 1 - (1 - I)^{\gamma_n}.
    \label{eq:mapping_function}
\end{equation}
with $\gamma_n$ as a random number whose logarithm value ${X_n = \log(\gamma_n)}$ is sampled as follows: $X_n \sim U(0, 3)$ for under-exposed reference images and $X_n \sim U(-2, 0)$ for over-exposed reference images


% with $\gamma_n$ is a randomly sampled vector with 3 elements, one for each channel, whose logarithm values as follows:
% \begin{equation}
% \log(\gamma_n) = [X_n + Z_n^r, X_n + Z_n^g, X_n + Z_n^b]^T
%     \label{eq:random_range}
% \end{equation}

% 
% where $Z_n^r, Z_n^g, Z_n^b \sim U(-0.5, 0.5)$, $X_n \sim U(0, 3)$ for under-exposed reference images and $X_n \sim U(-1, 0)$ for over-exposed reference images.


% At this stage, we empirically found that, applying the gamma function on the inverted image or not does not affect much on the final result. Nevertheless, since we want our tone mapping function at this module consistent with the tone mapping function in the enhancement network, which is described in \cref{enhancement_net}, taking the negative image as input has more advantage. 
As shown in Figure~\ref{fig:mapping}, learning the mapping function on the inverted image makes our training more stable than learning directly on the original image. In addition, our proposed function also has the same form as the well-known mathematical image processing model LIP~\cite{Jourlin2001LogarithmicIP}. This model had been proven with both physical and human visual systems, thus making our mapping function more theoretically sound.

\begin{figure}[]
\centering
\includegraphics[width=.45\textwidth, page=3]{image/figure.pdf}
\caption{The influence of the mapping function. Our training is more stable when we learn the mapping function on the inverted picture rather than the original image.}
\label{fig:mapping}
\vspace{-10pt}
\end{figure}

\subsection{Pseudo Ground-truth Image Generator}
\label{sec:pseudo_gt_generator}
To create the pseudo ground-truth image, we compare and combine the $2N$ generated reference images, the original image, and the enhancement network's output of the same image in the previous epoch.
The idea behind our approach is inspired by prior work on exposure fusion~\cite{mertens2007exposure}, in which a set of perceptual quality measures for each pixel are calculated in the reference image sequence. These measurements can encode desired attributes such as brightness, contrast, and saturation and has been shown their effectiveness in generating a high quality HDR (high dynamic range) image from an exposure sequence. Therefore, in this paper we adopt and customize these measurement scores as follow:

\noindent\textbf{Well-exposedness} estimates how likely it is that a pixel belongs to a well-exposed region. We use the L1 distance between the average intensity value of a local region to the well-exposed level, which is set to 0.5. Thus, the well-exposedness of a pixel is defined as 
\begin{equation}
    E(x,y) = \left| \mu_{p_{xy}} - 0.5 \right|
\end{equation}
where $p_{xy}$ is a patch $K \times K$ centered at $(x,y)$ and  $\mu_{p_{xy}}$ is its mean intensity value. We set $K=25$ in this paper.

\noindent\textbf{Local contrast} is the local variance of all pixels $I(u,v)$ of the patch $p_{x,y}$ \cite{ssim}
\begin{equation}
    C(x,y) = \dfrac{1}{K \times K}\sum_{u,v \in p_{x,y}}\left[I(u,v) - \mu_{p_{xy}}\right]^2
\end{equation}

\noindent\textbf{Color saturation} of a pixel measures its vividness. We use the saturation channel in HSV space to measure the color saturation of a pixel. In this color space, the saturation is defined as
% 
\begin{equation}
    S(x,y) = \dfrac{\max(R, G, B) -  \min(R, G, B)}{\max(R, G, B)}
\end{equation}
with $R, G, B$ corresponding to red, green and blue values of the pixel $(x,y)$.

Since a good looking output image is one with low well-exposedness value but high contrast and saturation values, we obtain the final pseudo-ground-truth image $T$ by combining these scores from all reference images $n$ as follows:
\begin{equation}
    
    T(x,y) = \max_{n=1..2N+2} \frac{C_n(x,y)S_n(x,y)}{E_n(x,y)}
\end{equation}

% Each pixel in the final pseudo-ground-truth image is taken from the same location of the reference image whose $Q$ score is the maximum among the reference images. 
% % Based on these matrix scores, for each position $(x, y)$ the value of reference whose score is highest is taken and combined to create the final ground-truth image.
% \begin{equation}
%     T(x,y) = \max{Q_i(x,y)}
% \end{equation}







\subsection{Image Enhancement Network} \label{enhancement_net}
% \begin{figure}[t]
% \centering
% % \captionsetup{scale=0.5\linewidth}
% \includegraphics[width=0.47\textwidth, page=4]{image/figure.pdf}
% \caption{Image enhancement module in detail. A lightweight UNet architecture is employed to predict the coefficient map $\gamma$ for each channel. The enhanced image is obtained by applying the gamma mapping function with the predicted coefficient map.}
% \label{fig:phase}
% \vspace{-5pt}
% \end{figure}


Similar to \cite{zerodce}, our network will learn to predict the intermediate parameter of a tone mapping function instead of directly predicting the output image. We design our lightweight enhancement network based on the UNet architecture~\cite{ronneberger2015unet}. To produce only positive gamma estimation, we take the absolute value of the output instead of using ReLU activation to avoid the dying ReLU problem while still achieving low computational cost. The detail of network architecture is provided in the \textit{Supplementary}. For consistency with the reference generation module, the invert gamma mapping function in \cref{refence_generator} is used to produce the final image $Y$ given the predicted gamma map $\gamma$ and the original image I: 
\begin{equation}
    Y = 1 - (1-I)^{\gamma}
\end{equation}
% 
We then train our model end-to-end to minimize following loss function:
$$L = L_{rec} + \alpha L_{tv}$$
where $L_{rec}$ and $L_{tv}$ are the reconstruction loss and total variation loss, respectively, and $\alpha$ is a coefficient to balance between the two losses.

\noindent\textbf{Reconstruction loss.} We adopt the mean squared error between the network prediction and the pseudo-ground-truth image as follows:
\begin{equation}
    L_{rec} = \dfrac{1}{3HW} \sum_{c \in {R, G, B}}\sum_{x,y}\left[(\hat{Y}(c,x,y) - T(c,x,y)\right] ^ 2
\end{equation}
% 
where $\hat{Y}$ is the output image and $T$ is our generated pseudo-ground-truth image in Sec.~\ref{sec:pseudo_gt_generator}; $H$, and $W$ are the height and width of the input image, respectively.

\noindent\textbf{Total variation loss.} In the homogeneous areas, the adjacent gamma values should be similar to avoid sudden changes, which can create visual artifacts. Therefore, we apply a familiar smoothness prior in image restoration tasks, called total variation minimization~\cite{Rudin1992NonlinearTV, Ng2011ATV}, to the estimated gamma map. The total variation loss is defined in equation \eqref{eq:tv_loss} 
%
\begin{equation}
\mathcal{L}_{tv} = \frac{1}{HW}\sum_{c \in \{R, G, B\}}(\nabla_x \log \gamma_c + \nabla_y \log \gamma_c),
    \label{eq:tv_loss}
\end{equation}
%
where $\gamma_c$ is the predicted gamma value corresponding to channel $c$, and $\nabla_x$ and $\nabla_y$ are the gradient operators in the horizontal and vertical directions of the predicted gamma map, respectively.





==> sections/4_experiment.tex <==



\section{Experiments}


\subsection{Experimental Setup}






\noindent\textbf{Datasets.} 
We assess our approach as well as comparative methods on two main multi-exposure datasets: Afifi (introduced by Afifi \etal{}~\cite{afifi2021learning}) and SICE~\cite{sice} datasets. The Afifi dataset contains 24,330 sRGB images rendered from the MIT-Adobe FiveK dataset \cite{fivek} by varying their digital exposure settings. The SICE dataset has two parts 1 and 2 with 360 and 229 multi-exposure sequences (set of images of the same scene captured at different exposure levels), respectively. We employ part 1 as the training set and part 2 as the test set. For generalization evaluation, we also test all approaches on the LOL dataset~\cite{retinexnet}, which is composed of 500 pairs of low-light and normal images.

% For SICE~\cite{sice} test set, we use our lighting classifier to divide the original testing set into two subsets: under-exposure (1104 images) and over-exposure (675 images) since the information about exposure value is not available.

\noindent\textbf{Implementation details.} We train our image enhancement network on an NVIDIA A100 GPU, using the Adam optimizer with the batch size of 64. In SICE dataset, our model is trained with 140 epochs while the number of epochs for training Afifi dataset is 30. The learning rate is 0.0005 and is reduced by half on plateau with the patience of 5. All the input images are resized to $256\times 256$ during training. The number of randomly generated reference is 2.  The coefficient of the total variation loss $\alpha$ for training on each dataset and other implementation details are empirically selected and reported in the \textit{Supplementary material}.


\subsection{Comparison with Prior Work}
We compare our approach with two non-learning methods: CLAHE \cite{clahe}, IAGCWD \cite{IAGCWD}, one unpaired method EnlightenGAN \cite{enlightengan}, two unsupervised methods: ZeroDCE~\cite{zerodce}, Zheng and Gupta~\cite{semanticguided}, and two supervised methods: HDRNet~\cite{hdrnet}, Afifi \etal{}~\cite{afifi2021learning}. The results of these methods are reproduced by using their public source codes with the recommended parameters. 

\noindent\textbf{Objective image quality assessment.} We adopt two standard referenced metrics: peak signal-to-noise ratio (PSNR) and structural similarity index measure (SSIM) in the cases where the ground-truth images are available in the testing set (for evaluation purposes only). To see the effectiveness of our method on each type of lighting condition, we also report the metric scores on lighting-dependent subsets of Afifi dataset, which includes 3,543 over-exposed images and 2,362 under-exposed images~\cite{afifi2021learning}. 

Table \ref{table:quantity_result} reports the quantitative results obtained by each method on the Afifi, SICE and LOL datasets. On the Afifi dataset, our approach outperforms all state-of-the-art unsupervised models include EnlightenGAN~\cite{enlightengan}, ZeroDCE~\cite{zerodce}, and ZeroDCE++~\cite{dce_extension} with significant margins (+5 and +0.1 in PSNR and SSIM metrics, respectively). On the SICE dataset, our approach also surpasses all other unsupervised methods on the SICE dataset with large margins (+3 and +0.02 in PSNR and SSIM metrics, respectively). When  comparing with other supervised methods, surprisingly, the proposed method obtains better results than HDRNet~\cite{hdrnet} and Afifi \etal{}~\cite{afifi2021learning} in SSIM index. 

\begin{table}
% \setlength{\tabcolsep}{5pt}
\small
\centering
\begin{tabular}{l|cc|cc|cc|cc|cc}
\hline
\multirow{3}{*}{\textbf{Method}} & \multicolumn{6}{c|}{\textbf{Afifi}} & \multicolumn{2}{c|}{\multirow{2}{*}{\textbf{SICE}}} & \multicolumn{2}{c}{\multirow{2}{*}{\textbf{LOL}}}  \\
 \cline{2-7}
 & \multicolumn{2}{c|}{Under} & \multicolumn{2}{c|}{Over} & \multicolumn{2}{c|}{Full} & \multicolumn{2}{c|}{} \\
 \cline{2-11}
 & PSNR & SSIM & PSNR & SSIM & PSNR & SSIM & PSNR & SSIM & PSNR & SSIM \\
\hline
CLAHE  (N)  & 16.67 & 0.780 & 18.19 & 0.806 & 17.58 & 0.796 & 13.89 & 0.610 & 10.02 & 0.427\\
IAGCWD  (N)  & 13.23 & 0.681 & 17.99 & 0.820 & 16.08 & 0.765  & 14.09 & 0.635 & 11.26 & 0.519 \\
\hline
HDRNet (S) & \textbf{19.35} & 0.817 & \textbf{20.65} & 0.846 & \textbf{20.13} & 0.834  &\underline{17.25}  &\underline{0.683}  & \textbf{17.29} & \textbf{0.766}  \\
Afifi \etal{} (S) & \underline{18.88} & \underline{0.845} & {19.05} & \underline{0.850} & {18.98} & \underline{0.848}  & - & - & - & -\\
\hline
ZeroDCE (U) & 15.36 & 0.783 & 11.85 & 0.739 & 13.25 & 0.757  & 14.28 & 0.657 & 14.16 & 0.654\\
Zheng and Gupta (U)  & 16.69  & 0.806 & 11.58 & 0.726 & 13.62 & 0.758 & 12.54 & 0.626 & 14.89 & 0.675\\
EnlightenGAN (U*) & 14.28 & 0.752 & 14.05 & 0.766 & 14.14 & 0.762  &	14.60 &	0.680 & 12.32 & 0.596 \\
\hline
% \Approach~(U)  & \underline{18.98} & \textbf{0.859} & 18.77 & \textbf{0.863} & 18.86 & \textbf{0.863} & \underline{17.11} & \textbf{0.708} & \underline{15.92} & \underline{0.676}\\
\Approach~(U)  & 18.82 & \textbf{0.858} &\underline{19.72} & \textbf{0.875} &\underline{19.36} & \textbf{0.869} & \textbf{17.74} & \textbf{0.704} & \underline{16.60} & \underline{0.693} \\
\end{tabular}
%\vspace{-5pt}
\caption{Results on SICE, Afifi and LOL dataset. The higher the better. The terms ``under" and ``over" stand for under-exposure and over-exposure subsets. The terms ``N", ``U", ``U*" ``S" stand for non-learning, unsupervised, unpaired, and supervised respectively. Due to Matlab license issue, we could not train and evaluate performance of Afifi \etal{} on SICE and LOL dataset. }
\label{table:quantity_result}
%\vspace{-5pt}
\end{table}

We further assess the generalization abilities of all methods on the LOL dataset. In this experiment, we report results of all methods trained on SICE dataset without further tuning. As can be seen in Table~\ref{table:quantity_result}, the same trend can be observed in which we outperform all unsupervised and unpaired approaches and perform slightly worse than a supervised model HDRNet~\cite{hdrnet}. However, HDRNet~\cite{hdrnet} tends to produce output images with visual artefacts that are shown in the next section. 

% Compared with unsupervised and non-learning methods,
% , our model is the only one that works on both under-exposure and over-exposure. Specifically, CLAHE~\cite{clahe} gives a good output in the over-exposure case, but it fails in the under-exposure case. Meanwhile, ZeroDCE~\cite{zerodce} and EnlightenGAN~\cite{enlightengan} produce output images quite well in the under-exposure case, but they seem to fail to recover the details of the image in the over-exposure cases. 

\noindent\textbf{Subjective image quality assessment.} 
Visual comparison among unsupervised approaches on typical under-exposure and over-exposure scenes are presented in Figure \ref{fig:visual_unsupervised}. Our model is the only one that works on both under- and over-exposure. CLAHE~\cite{clahe}, in particular, produces good results in the over-exposure situation but fails in the under-exposure cases. ZeroDCE~\cite{zerodce} and EnlightenGAN~\cite{enlightengan} produce good output images in the under-exposure situation, but they appear to fail to recover the image's details in the over-exposure condition.
Visual comparison on typical under-exposure and over-exposure scenes are presented in Figure \ref{fig:visual_supervised}. As we mentioned in the previous, although HDRNet~\cite{hdrnet} achieved the best PSNR and SSIM scores in most of the cases, however, it often produces output images with visible artifacts (shown in Figure~\ref{fig:visual_supervised}).

\begin{figure}[t]
\includegraphics[width=.48\textwidth, page=7]{image/figure.pdf}
\caption{Results of user study - Others vs Ours. The blue color shows the preference percentages of the other methods, while the orange color shows ours.}
\label{fig:user_study}
\end{figure}

\noindent\textbf{User study.} For more convincing evaluation, we also conduct a user study with 135 participants on 30 scenes from the testing set to assess human preference on the enhanced results. For each scene, we show our enhanced image with another image which is a result of a random method. We restrict the sampling method to ensure that all method present evenly across user response.  The participants then are asked to pick a better image in each pair based on the three following criteria: (1) whether all parts in the image are clearly visible; (2) whether the result introduces any color deviation; and (3) the better image based on their preference. The detailed comparison between ours and other methods is reported in Figure~\ref{fig:user_study}. As can be seen, our enhanced images are preferred in all cases including both supervised and unsupervised approaches, only Afifi et al.'s approach~\cite{afifi2021learning}  has a preferable ration that is relatively comparable to ours. HDRNet~\cite{hdrnet} is less desirable in our user study due to their unpleasant output images. 




%\noindent\textbf{Visual qualitative assessment.} 

% \subsection{Computational Cost Comparison}
% We evaluate the computational cost of running our model on a mobile device with other methods. To measure the latencies, we convert all models to TFLite and run them on a Samsung Tab S6 through TFLite Benchmark Tool, except HDRNet \cite{hdrnet}, and the model proposed by Afifi \etal{} \cite{afifi2021learning} because they require Bilateral Guided Upsampling \cite{bgu} which is difficult for us to obtain an efficient version for mobile. The runtime is average on 20 pre-processed images of size $1080 \times 720$. We also report the number of multiply–accumulated operations (MACs) and the number of trainable parameters for each network in Table \ref{table:Computational_performance}. As we can see, our method achieves the fastest runtime, which is 3.9 and 6.4 times faster than  Zheng and Gupta~\cite{semanticguided} and ZeroDCE, respectively. Our tiny network with only 5,023 parameters and 0.69 GMACs is so lightweight that it is very suitable for real-time applications.

\begin{figure*}[ht]
\centering
\includegraphics[width=\textwidth, page=5]{image/figure.pdf}
\caption{Visual comparison with unsupervised and non-learning methods. The first and third rows show the whole images, while the second and last rows show the corresponding close-ups. Only our method works in both under- and over-exposure situations. CLAHE~\cite{clahe} performs well in over-exposure situations but poorly in under-exposure situations. While ZeroDCE~\cite{zerodce} and EnlightenGAN~\cite{enlightengan} generate decent output images in the under-exposure cases, they fail to handle the image's features in the over-exposure situations.}
\label{fig:visual_unsupervised}
\end{figure*}



\begin{figure*}[ht]
\centering
\includegraphics[width=\textwidth, page=6 ]{image/figure.pdf}
\caption{Visual comparison with supervised methods. The first and third rows show the whole images, while the second and last rows show the corresponding close-ups. Although HDRNet~\cite{hdrnet} achieved the best PSNR and SSIM scores in most of the cases, it often produces output images with visible artifacts.}
\label{fig:visual_supervised}
\vspace{-5pt}
\end{figure*}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Ablation Study} 





% \begin{figure*}[]
% \centering
% \includegraphics[width=1.0\textwidth, page=10]{image/images.pdf}
% \caption{Ablation study of the contribution of each loss function on the quality of the output image. From left to right are exposure loss  $\mathcal{L}_{exp}$, contrast preserving loss $\mathcal{L}_{contrast}$, total variation loss $\mathcal{L}_{tv}$, and color constancy loss $\mathcal{L}_{col}$.}
% \label{fig:loss_fn}
% \vspace{-10pt}
% \end{figure*}


%%%%%%%%%%%%%%%%%%%%%%




In this section, we conduct experiments on analyzing the impact of different components of our proposed framework, including the pseudo GT generator branch and the loss functions. We then go in detail and analyze the impact of each component in the pseudo GT branch, including the way to sample random references and whether to add previous prediction to the set of reference images.

\noindent\textbf{Pseudo GT generator.}
We first analyze the influence of pseudo GT generator by replacing our Enhancement Network with the network presented in ZeroDCE~\cite{zerodce} and  EnlightenGAN~\cite{enlightengan}, and retrain these models on the SICE dataset. As demonstrated in Table~\ref{table:pseudo_GT}, using our proposed framework makes these two networks deal with the over-exposure cases better, thus significantly improving their overall performance on SICE dataset (+1 in PSNR). Qualitative results are provided in the \textit{Supplementary material}.

\begin{table}[t]
\centering
\begin{tabular}{lcccc} 
\hline
\textbf{Method} & \textbf{PSNR} & \textbf{SSIM}\\ 
\hline
ZeroDCE~\cite{zerodce} & 14.28 & 0.657\\
ZeroDCE~\cite{zerodce} with pseudo GT & 15.30 & 0.672 \\
\hline
EnlightenGAN~\cite{enlightengan} & 14.60 & 0.680\\
EnlightenGAN~\cite{enlightengan} with pseudo GT & 15.34 & 0.657 \\
\end{tabular}
\caption{The influence of pseudo GT generator on ZeroDCE~\cite{zerodce} and EnlightenGAN~\cite{enlightengan} on the SICE dataset. Our suggested approach also improves these two networks' abilities in handling over-exposure cases, resulting in a considerable improvement (+1 in PSNR).}
\label{table:pseudo_GT}
\vspace{-1pt}
\end{table}
% Move to suppementary material

\begin{figure}[t]
\includegraphics[width=.48\textwidth, page=11]{image/figure.pdf}
\vspace{-10pt}
\caption{The impact of range to sample random reference. $U(a;b)$ indicates range to sample brightness factor $X$.}
\label{fig:Random_range}
\end{figure}

\noindent\textbf{Impact of range to sample references.}
%idea: top 3 rows for brightness modification, last 4 rows for color manipulation.
In terms of brightness modification, we found that the best range to sample the reference images is from 0 to 3 for darker image generation and from -2 to 0 for synthesizing brighter images. 
If we narrow the range for under-exposure to $(0,2)$, our model's performance decrease noticeably. The reason is that the produced gamma map is then limited, thus, our model could not increase the brightness of the input image to a proper value in extreme cases, as demonstrated in the second rows of Figure~\ref{fig:Random_range}. 
% If we narrow the range to sample reference images to $(-1, 1)$ our model's performance decrease significantly as shown in Table~\ref{table:Random_range}. The reason is that the produced gamma map is then limited, thus, our model could not increase the brightness of the input image to a proper value in extreme cases, as demonstrated in the second rows of Figure~\ref{fig:Random_range}. 
On the other hand, when it comes to the range of sampling brighter images, extending this range from $(-2, 0)$ to $(-3, 0)$ might create undesired artifacts in overexposed areas. Due to image clipping, the color information in these areas is not well preserved. Therefore, when reducing image brightness, instead of producing a vivid image, our model tends to modify the color tone of the input image to gray, which is visually unpleasant.
We also conduct experiments to see if incorporating color manipulation into the reference generation process can help our model improve the color in output images. In particular, we replace the random gamma value $\gamma_n$ shared between all color channels to  vector with 3 elements, whose logarithm values as follows:
\begin{equation}
\log(\gamma_n) = [X_n + Z_n^r, X_n + Z_n^g, X_n + Z_n^b]^T
    \label{eq:random_range}
\end{equation}
The experimental results are reported in the last three rows of Table~\ref{table:Random_range}.
% When the range to sample color. 
It seems that using color perturbation in reference images has little effect on the performance of our enhancement network. 
% We report the quantitative score of our approach trained on SICE dataset with different reference sampling range in Table~\ref{table:Random_range}. In terms of only modifying brightness of image (results are shown in the top 3 rows of Table~\ref{table:Random_range}), when the range to sample is too small, it limits the image modification, thus our model could not enhance image extreme cases, for example, the scence in second row of Figure~\ref{fig:Random_range}. On the other hand, extending the range to sample brighter image from $(-1, 0)$ to (-3, 0)) might create undesired artifact in overexposed cases.
% We also try to sample the gamma value of each channel differently to see its effects. Specifically, instead of using only one gamma value $\gamma_n$ for all channels, we sample a vector with 3 elements, one for each channel, whose logarithm values as follows:
% \begin{equation}
% \log(\gamma_n) = [X_n + Z_n^r, X_n + Z_n^g, X_n + Z_n^b]^T
%     \label{eq:random_range}
% \end{equation}
% As can be seen from the last four rows of Table~\ref{table:Random_range}, generating reference with color modification does not have much impact to the performance of our enhancement network.


\begin{table}[t]
\centering
\begin{tabular}{lcccc} 
\hline
\textbf{Method} & \textbf{PSNR} & \textbf{SSIM}\\ 
\hline
%$X_n \sim U(-1, 1)$ & 15.42 & 0.643 \\
$X_n \sim U(-2, 2)$ & 17.20 & 0.690 \\
$X_n \sim U(-2, 3)$  & 17.74 & 0.704  \\
$X_n \sim U(-3, 3)$ & 17.80 & 0.703  \\
\hline
Without color perturbation & 17.74 & 0.704  \\
$Z_n^r, Z_n^g, Z_n^b \sim U(-0.1, 0.1)$  & 17.79 & 0.704  \\
$Z_n^r, Z_n^g, Z_n^b \sim U(-0.5, 0.5)$ & 17.52 & 0.701 \\
%$Z_n^r, Z_n^g, Z_n^b \sim U(-1, 1)$  & 17.09 & 0.703  \\
\end{tabular}
\caption{The impact of range to sample random reference to the final model performance on SICE~\cite{sice} dataset with $X_n$ for brightness modification and $Z_n^r, Z_n^g, Z_n^b$ for color modification. }
\label{table:Random_range}
\vspace{-10pt}
\end{table}



\noindent\textbf{Adding previous prediction to the set of reference images.} 
To examine the influence of the proposed training strategy on the whole training process, we retrain our network for 40 epochs with and without taking the previous prediction as a reference, then record the performance of our model on the SICE test set after each epoch. The results are plotted in Figure~\ref{fig:adding_previous_output}. By adding the previous output to the reference set, our model converges faster and achieves higher metric scores. More specifically, in the case of using the previous output as a reference, the final metric scores increase approximately $+1.5$ and $+0.02$ in terms of PNSR and SSIM, respectively in compared with the absence of previous output.

\noindent\textbf{Contribution of total variation loss.} We also present the results of our enhancement network trained with the absence of total variation loss in Figure~\ref{fig:tv_loss}. Without this loss, our model tends to break the relation between neighboring regions, resulting in an image with apparent artifacts.
\begin{figure}[t]
\includegraphics[width=.48\textwidth, page=15]{image/figure.pdf}
\caption{Our model's performance with and without adding previous output to reference set, respect to first 40 epochs. By adding previous output to reference set, our model convergence faster and achieve  higher metric scores. }

\label{fig:adding_previous_output}
\end{figure}
\begin{figure}[t]
\includegraphics[width=.48\textwidth, page=8]{image/figure.pdf}
\vspace{-15pt}
\caption{The influence of total variation loss. The left-top corners show the corresponding close-ups. Without this loss, the gamma values of neighboring regions are not smooth that results in an image with visible artifacts.}

\label{fig:tv_loss}
\end{figure}


% \begin{table}[t]
% \centering
% \begin{tabular}{lcccc} 
% \hline
% {{\textbf{Method}}} & \textbf{PSNR} & \textbf{SSIM}\\ 
% \hline
% Our method & 17.11 & 0.708 \\
% %\hline
% Without taking model output as reference  & 16.28 & 0.696 \\
% %Without total variation loss & 16.68 & 0.699 \\

% \end{tabular}
% \caption{The impact of different components to the final performance on SICE~\cite{sice} dataset.}
% \label{table:Random_reference}
% \vspace{-1pt}
% \end{table}








==> sections/5_application.tex <==
% \section{Applications}


% % \label{application}
% % \begin{figure}[]
% %     \centering
% %     \includegraphics[scale=0.35]{image/plot_pr.png}
% %     \includegraphics[scale=0.14, page=16]{image/images.pdf}
% %     \vspace{-5pt}
% %     \caption{Top: Precision-recall curve for face detection in the dark. Bottom: Outputs of the detection model of before and after preprocessed images by our method.}
% %     \label{fig:pr_curve}
% %     \vspace{-10pt}
% % \end{figure}

% In this section, we evaluate the efficiency of our method when it is used as a preprocessing module in the face detection task.
% Experiments are conducted on the training and validation set of DARK FACE dataset \cite{9049390, retinexnet} composed of 6,000 images captured in low-light environments. We use Dual Shot Face Detector (DSFD) \cite{dsfd}, trained on WIDER FACE dataset as the baseline model. More concretely, we feed the images enhanced by several low-light image enhancement methods to the pretrained DFSD model and observe how its performance changes. Figure \ref{fig:pr_curve} illustrates the precision-recall curve and the average precision computed by the evaluation tool provided in DARK FACE dataset \cite{9049390, retinexnet} when applying different image enhancement approaches. Preprocessing images by low-light image enhancement methods significantly increases the precision of the face detector compared with using raw images. Our method achieves a comparable result with ZeroDCE and ZeroDCE++ while having a much lower computational cost. The results in Figure \ref{fig:pr_curve} also demonstrate the efficiency of our method. It lights up the faces in extremely dark regions, thus improves the performance of the DFSF.
% % Specifically, we conduct experiments on two face datasets: DARK FACE dataset \cite{9049390, retinexnet} and our synthetic dataset. The former is composed of 10000 images captured in low-light environments. The latter is rendered by varying gamma values from the FDDB dataset \cite{fddb} to simulate a wider range of brightness distortion. We use Dual Shot Face Detector (DSFD) \cite{dsfd}, trained on the WIDER FACE dataset as the baseline model. 

% % \noindent\textbf{Results on DARK FACE dataset.} Experiments are performed on the training and validation set of the DARK FACE dataset due to the non-public bounding boxes of the test set. More concretely, we feed the images enhanced by several low-light image enhancement methods to the DFSD model and observe how its performance changes. Figure \ref{fig:pr_curve} illustrates the precision-recall curve and the average precision computed by the evaluation tool provided in DARK FACE dataset \cite{9049390, retinexnet} when applying different image enhancement approaches. As depicted in Figure \ref{fig:pr_curve}, preprocessing images by low-light image enhancement methods significantly increases the precision of the face detector compared with using raw images. Our method achieves a comparable result with ZeroDCE and ZeroDCE++ while having a much lower computational cost. The example shown in Figure \ref{fig:pr_curve} also demonstrates the efficiency of our method. It lights up the faces in extremely dark regions, thus improves the performance of the DFSF.  


% % \khoi{Need presentation and some discussions here. Be consistent with the name of our approach}


==> sections/6_conclusion.tex <==
\section{Conclusion}
 \begin{figure}[]
    \centering
    \includegraphics[width=.48\textwidth, page=10]{image/figure.pdf}
    \caption{Failure examples of correcting (left) under-exposure and (right) over-exposure images. The first row shows the whole images, while the second row shows the corresponding close-ups. }
    \label{fig:failuer_case}
    \vspace{-10pt}
\end{figure}
We have introduced a novel progressive self-enhancement network for image enhancement that is robust to a variety of severe lighting circumstances, including under-exposure and over-exposure. In particular, we have developed a new method for generating effective pseudo-GT images for training our extreme-light enhancement network in an unsupervised manner. As a result, the burden of gathering the matched photographs is removed.
Our extensive experiments show that the proposed approach consistently outperforms previous unsupervised methods by large margins on several public datasets and obtains comparable results with supervised counterparts. 


Similar to the prior methods, our approach still has some drawbacks due to severe data loss issues. As shown in the left part of Figure~\ref{fig:failuer_case}, our method may introduce noise when enhancing the extreme dark region where the signal to noise ratio is too low. Furthermore, our method may fail at recovering the detail in an entirely saturated area (as shown in the right part of Figure~\ref{fig:failuer_case}). However, other approaches also encounter difficulties in these challenging conditions. 

%In the future, we intend to examine how to extend our model for videos where temporal consistency is critical.

